Cubic Dirac Operators and Dirac Cohomology for Basic Classical Lie Superalgebras

We study the Dirac cohomology of supermodules over basic classical Lie superalgebras, formulated in terms of cubic Dirac operators associated with parabolic subalgebras. Specifically, we establish a super-analog of the Casselman-Osborne theorem for supermodules with an infinitesimal character and use it to show that the Dirac cohomology of highest-weight supermodules is always non-trivial. In particular, we explicitly compute the Dirac cohomology of finite-dimensional simple supermodules for basic Lie superalgebras of type 1 with a typical highest weight, as well as of simple supermodules in the parabolic BGG category. We further investigate the relationship between Dirac cohomology and Kostant (co)homology, proving that, under suitable conditions, Dirac cohomology embeds into Kostant (co)homology. Moreover, we show that this embedding lifts to an isomorphism when the supermodule is unitarizable.

==> hacks.tex <==
\makeatletter

%%%%%% draftcontrol
%%%%%%

\expandafter\ifx\csname draftcontrol\endcsname\relax\global\def\draftcontrol{0}  
\fi 

{\count255=\time\divide\count255 by 60 
\xdef\hourmin{\number\count255} 
\multiply\count255 by-60\advance\count255 by\time 
\xdef\hourmin{\hourmin:\ifnum\count255<10 0\fi\the\count255}} 
\def\draftdate{\number\month/\number\day/\number\year\ \ \ \hourmin } 

\def\@version#1{%
  \ifnum\draftcontrol=1 
  \typeout{}\typeout{#1}\typeout{} 
  \vskip3mm\centerline{%
    \hbox{%
      \fbox{\normalsize{\tt DRAFT -- #1 -- }%
          {\draftdate}}}}\vskip3mm 
\fi} 
\let\version\@version 


%%%
%%%%%% More space in Abstract an Tableofcontents
%%%%%%%%%

\renewenvironment{abstract}{%
  \ifx\maketitle\relax
    \ClassWarning{\@classname}{Abstract should precede
      \protect\maketitle\space in AMS document classes; reported}%
  \fi
  \global\setbox\abstractbox=\vtop \bgroup
    \normalfont\Small
    \list{}{\labelwidth\z@
      \leftmargin3pc \rightmargin\leftmargin
      \listparindent\normalparindent \itemindent\z@
      \parsep\z@ \@plus\p@
      \let\fullwidthdisplay\relax
    }%
    \item[\hskip\labelsep\scshape\abstractname.]%
}{%
  \endlist\egroup
  \ifx\@setabstract\relax \@setabstracta \fi
}

%%%
%%%%%% small big symbols
%%%%%%%%%

\newcommand{\makesmalleroperator}[1]{%
  \expandafter\let\csname saved\string#1\endcsname#1% save the old command
  \def#1{\mathop{\small@mathchoice#1}}% redefine it
}
\def\small@mathchoice#1{%
  \mathchoice{\text{\raisebox{0.25ex}{\scalebox{0.8}{$\@nameuse{saved\string#1}$}}}}%
             {\@nameuse{saved\string#1}}%
             {\@nameuse{saved\string#1}}%
             {\@nameuse{saved\string#1}}%
}

\makesmalleroperator\bigwedge
\makesmalleroperator\bigoplus
\makesmalleroperator\bigotimes




%%%
%%%%%% horizontal lines in arrays
%%%%%%%%%

\newcommand\tstrut{\rule[0ex]{0pt}{2.2ex}}

%%%

%%%
%%%%%% margin notes
%%%%%%%%%

\def\revise#1{\raisebox{-0em}{\rule{3pt}{1em}}% 
              \marginpar{\raisebox{.5em}{\vrule width3pt\ 
               \vrule width0pt height 0pt depth0.5em 
                \hbox to 0cm{\hspace{1.4cm}{% 
                \parbox[t]{5em}{\raggedright\footnotesize{#1}}}\hss}}}} 

%%%
%%%%%% Bibliography
%%%%%%%%%

%%% this saves a bit of space
\renewcommand*{\bibsetup}{%
  \interlinepenalty=5000\relax
  \widowpenalty=10000\relax
  \clubpenalty=10000\relax
  \raggedbottom
  \frenchspacing
  \biburlsetup
  \renewcommand\baselinestretch{1}
}
\renewcommand{\bibfont}{\fontsize{9pt}{11pt}\selectfont}
\setlength\bibitemsep{.1em}
\setlength\bibhang{0em}
\setlength\biblabelsep{.7em}

%%% this suppresses the In: 
\renewbibmacro{in:}{}
\DeclareFieldFormat{doilink}{%
  \iffieldundef{doi}%
  {#1}%
  {\href{https://doi.org/\thefield{doi}}{#1}}
}
%%% and puts doi link around journal reference
%%% (hacked from standard.bbx https://ctan.org/tex-archive/macros/latex/contrib/biblatex/latex/bbx?lang=en)
\DeclareBibliographyDriver{article}{%
  \usebibmacro{bibindex}%
  \usebibmacro{begentry}%
  \usebibmacro{author/translator+others}%
  \setunit{\printdelim{nametitledelim}}\newblock
  \usebibmacro{title}%
  \newunit
  \printlist{language}%
  \newunit\newblock
  \usebibmacro{byauthor}%
  \newunit\newblock
  \usebibmacro{bytranslator+others}%
  \newunit\newblock
  \printfield{version}%
  \newunit\newblock
  \usebibmacro{in:}
  \iffieldundef{journaltitle}
   {\printtext[journaltitle]{Preprint} \mkbibparens{\printdate}}
   {\printtext[doilink]{%
    \usebibmacro{journal+issuetitle}%
    \newunit
    \usebibmacro{byeditor+others}%
    \newunit
    \usebibmacro{note+pages}%
    \newunit\newblock
    \iftoggle{bbx:isbn}
      {\printfield{issn}}
      {}%
   }
   }
  \newunit\newblock
  \usebibmacro{doi+eprint+url}
  \newunit\newblock
  \usebibmacro{addendum+pubstate}%
  \setunit{\bibpagerefpunct}\newblock
  \usebibmacro{pageref}%
  \newunit\newblock
  \iftoggle{bbx:related}
    {\usebibmacro{related:init}%
     \usebibmacro{related}}
    {}%
  \usebibmacro{finentry}}

%%% this puts brackets around arxiv if journal exists
\letbibmacro{nakedEprint}{eprint}
\renewbibmacro*{eprint}{%
  \iffieldundef{eprint}
    {}
    {\iffieldundef{journaltitle}
      {\usebibmacro{nakedEprint}}
      {\printtext{{\usebibmacro{nakedEprint}}}}} %\mkbibbrackets I think there are too many brackets
}
%%% and changes format of [eprint:arxiv]
%%% (hacked from: https://packages.oth-regensburg.de/ctan/macros/latex/contrib/biblatex/latex/biblatex.def)
\DeclareFieldFormat{eprint:arxiv}{%
  \ifhyperref
    {\href{https://arxiv.org/\abx@arxivpath/#1}{%
       \nolinkurl{arXiv:#1}%
       \iffieldundef{eprintclass}
         {}
         {\addspace{\mkbibbrackets{\thefield{eprintclass}}}}}}  %%% remmoved \texttt
    {\nolinkurl{arXiv:#1}%
     \iffieldundef{eprintclass}
       {}
       {\addspace{\mkbibbrackets{\thefield{eprintclass}}}}}}   %%% removed \texttt

\makeatother
